EMSx: a numerical benchmark for energy management systems

Inserting renewable energy in the electric grid in a decentralized manneris a key challenge of the energy transition. However, at local scale, both production and demand display erratic behavior, which makes it delicate to match them. It is the goal of Energy Management Systems (EMS) to achieve such balance at least cost. We present EMSx, a numerical benchmark for testing control algorithms for the management of electric microgrids equipped with a photovoltaic unit and an energy storage system. EMSx is made of three key components: the EMSx dataset, provided by Schneider Electric, contains a diverse pool of realistic microgrids with a rich collection of historical observations and forecasts; the EMSx mathematical framework is an explicit description of the assessment of electric microgrid control techniques and algorithms; the EMSx software EMSx.jl is a package, implemented in the Julia language, which enables to easily implement a microgrid controller and to test it. All components of the benchmark are publicly available, so that other researchers willing to test controllers on EMSx may reproduce experiments easily. Eventually, we showcase the results of standard microgrid control methods, including Model Predictive Control, Open Loop Feedback Control and Stochastic Dynamic Programming.

==> commandes.tex <==




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% COULEURS 
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newrgbcolor{Violet}{0.8 0.1 0.9}
% \newrgbcolor{Jaune}{1 1 0}
% \newrgbcolor{Lagon}{0 1. 1}
% \newrgbcolor{LemonChiffon}{0. 0.2 0.2}
% \newrgbcolor{LightBlue}{0.68 0.85 0.9}
% \newrgbcolor{darkblue}{0.1 0.1 1}
% \newrgbcolor{LucRed}{0.8 0.2 0.2}
% \newrgbcolor{myred}{0.8 0.2 0.2}

\newcommand{\noir}[1]{\textcolor{black}{#1}}
\newcommand{\noire}[1]{\textcolor{black}{#1}}
\newcommand{\rouge}[1]{\textcolor{red}{#1}}
\newcommand{\bleue}[1]{\textcolor{blue}{#1}}
\newcommand{\bleu}[1]{\alert{#1}}
\newcommand{\verte}[1]{\textcolor{green}{#1}}
\newcommand{\blanc}[1]{\textcolor{white}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% NOUVEAUX ENVIRONNEMENTS                                  %%%%%
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newenvironment{PETIT}{%
\small }%  
{\normalsize}

\newenvironment{Petit}{%
\footnotesize }%  
{\normalsize}

\newenvironment{petit}{%
\tiny }%
{\normalsize}

% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{remark}[theorem]{Remark}
\newtheorem{assumption}{Assumption}

 % \newenvironment{proof}{\small{\bf Proof.}}%
 % {\hfill$\Box$\normalsize\bigskip}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% GENERALITES %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\subsubsubsection}[1]{\paragraph{#1.}}
\newcommand{\subsubsubsubsection}[1]{\medskip\noindent\textit{#1}.}

\newcommand{\eqsepv}{\; , \enspace}       
\newcommand{\eqfinv}{\; ,}                
\newcommand{\eqfinp}{\; .}                
\newcommand{\eqfinpv}{\; ;}               
 
\newcommand{\ind}[1]{_{#1}}     % indice
\newcommand{\IND}[1]{(#1)}

\renewcommand{\bar}{\overline}
\renewcommand{\tilde}{\widetilde}
\newcommand{\transp}{^{\top}}
\newcommand{\upper}{^{\sharp}}
\newcommand{\llower}{^{\flat}}
\newcommand{\lloweropt}{^{\flat,\star}}

\newcommand{\wrt}{\text{w.r.t.}}                            % ``w.r.t.''
\newcommand{\IFF}{iff~} 
%\newcommand{\newblock}{}
\newcommand{\mtext}[1]{\,\mbox{#1}\,} %text in maths
%\newcommand{\text#1{\quad\mbox{#1}\quad} %wide text in maths
\newcommand{\ds}{\displaystyle}
%\newcommand{\eqref}[1]{(\ref{#1})}

\newcommand{\module}[1]{\left| #1 \right|}
\newcommand{\norm}[1]{\|#1\|}
% \newcommand{\norme}[1]{\|#1\|}
% \newcommand{\norm}[2]{\|#1\|_{#2}}
\newcommand{\defegal}{:=}
%\newcommand{\matrix}{M}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% Parenth\`{e}ses, crochets et accolades
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sequence}[2]{\left\{#1\right\}_{#2}}           % Suite
\newcommand{\proscal}[2]{\left\langle#1\:,#2\right\rangle}  % Produit scalaire
\newcommand{\bscal}[2]{\big\langle#1\:,#2\big\rangle}       % Produit scalaire

\newcommand{\doublecrochet}[1]{\llbracket #1 \rrbracket}    %{[[#1]]}

\newcommand{\np}[1]{(#1)}                                   % Parenth\`{e}se normal
\newcommand{\bp}[1]{\big(#1\big)}                           % Parenth\`{e}se big
\newcommand{\Bp}[1]{\Big(#1\Big)}                           % Parenth\`{e}se Big
\newcommand{\bgp}[1]{\bigg(#1\bigg)}                        % Parenth\`{e}se bigg
\newcommand{\Bgp}[1]{\Bigg(#1\Bigg)}                        % Parenth\`{e}se Bigg

\newcommand{\dc}[1]{[ \! [ #1 ] \! ]}                       % Double crochet
\newcommand{\nc}[1]{[#1]}                                   % Crochet normal
\newcommand{\bc}[1]{\big[#1\big]}                           % Crochet big
\newcommand{\Bc}[1]{\Big[#1\Big]}                           % Crochet Big
\newcommand{\bgc}[1]{\bigg[#1\bigg]}                        % Crochet bigg
\newcommand{\Bgc}[1]{\Bigg[#1\Bigg]}                        % Crochet Bigg

\newcommand{\na}[1]{\{#1\}}                                 % Accolade normal
\newcommand{\ba}[1]{\big\{#1\big\}}                         % Accolade big
\newcommand{\Ba}[1]{\Big\{#1\Big\}}                         % Accolade Big
\newcommand{\bga}[1]{\bigg\{#1\bigg\}}                      % Accolade bigg
\newcommand{\Bga}[1]{\Bigg\{#1\Bigg\}}                      % Accolade Bigg

\newcommand{\normdelim}[1]{\np{#1}}                         % Taille ``normal''
\newcommand{\bigdelim}[1]{\bp{#1}}                          % Taille ``big''
\newcommand{\Bigdelim}[1]{\Bp{#1}}                          % Taille ``Big''
\newcommand{\biggdelim}[1]{\bgp{#1}}                        % Taille ``bigg''
\newcommand{\Biggdelim}[1]{\Bgp{#1}}                        % Taille ``Bigg''
\newcommand{\vardelim}[1]{\left(#1\right)}                  % Taille ``variable''

\newcommand{\normdelims}[2]{\normdelim{#1\mid#2}}           % avec s\'{e}parateur
\newcommand{\bigdelims}[2]{\bigdelim{#1\ \big|\ #2}}        %
\newcommand{\Bigdelims}[2]{\Bigdelim{#1\ \Big|\ #2}}        %
\newcommand{\biggdelims}[2]{\biggdelim{#1\ \bigg|\ #2}}     %
\newcommand{\Biggdelims}[2]{\Biggdelim{#1\ \Bigg|\ #2}}     %
\newcommand{\vardelims}[2]{\vardelim{#1\mid#2}}             %



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% ENSEMBLES ET SYMBOLES
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\RR}{{\mathbb R}} %"ensemble des reels"   
\newcommand{\NN}{{\mathbb N}} %"ensemble des entiers naturels"  
\newcommand{\ZZ}{{\mathbb Z}} %"ensemble des entiers relatifs"  
\newcommand{\CC}{{\mathbb C}} 
\newcommand{\DD}{{\mathbb D}} 
\newcommand{\BB}{{\mathbb B}} %"symbole d'esperance mathematique"
\newcommand{\EE}{{\mathbb E}} %"symbole d'esperance mathematique"
\newcommand{\FF}{{\mathbb F}} %"symbole d'esperance mathematique"
\def\HH{\mathbb H} % et non pas \newcommand{\HH}{{\mathbb H}} 
\newcommand{\PP}{{\mathbb P}} %"symbole de probabilite"
\newcommand{\QQ}{{\mathbb Q}} %"symbole de probabilite"
\newcommand{\TT}{{\mathbb T}} 
\newcommand{\UU}{{\mathbb U}} 
\newcommand{\VV}{{\mathbb V}} 
\newcommand{\WW}{{\mathbb W}} 
\newcommand{\XX}{{\mathbb X}} 
\newcommand{\YY}{{\mathbb Y}} 
\newcommand{\1}{{\mathbf 1}}

\newcommand{\espace}[1]{\mathbb{#1}}                        % Espace de Hilbert
\newcommand{\espacea}[1]{\mathbb{#1}}                       % Espace d'arriv\'{e}e
\newcommand{\espacef}[1]{\mathcal{#1}}                      % Espace fonctionnel
\newcommand{\defset}[2]{\left\{#1\:\left|\:#2\right.\right\}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% THÉORIE DU CONTRÔLE 
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\control}{u}
\newcommand{\Control}{U}
\newcommand{\CONTROL}{{\mathbb U}} 

\newcommand{\state}{x}
\newcommand{\State}{X}
\newcommand{\STATE}{{\mathbb X}}

\newcommand{\uncertain}{w}
\newcommand{\Uncertain}{W}
\newcommand{\UNCERTAIN}{{\mathbb W}} 

\newcommand{\dynamics}{f}
%\newcommand{\Dynamics}{F}
\newcommand{\Dynamics}[2]{f_{#1:#2}}
\newcommand{\tildeDynamics}[2]{\tilde{f}_{#1:#2}}

% \newcommand{\Output}{\mathtt{Obs}}
% \newcommand{\output}{{\Violet y}}
% \newcommand{\output}{y}

%% Time

\newcommand{\horizon}{T}
\newcommand{\tinitial}{t_0}
\newcommand{\tinitialplusone}{\tinitial +1}
\newcommand{\tinitialplustwo}{\tinitial +2}
\newcommand{\tun}{r}
\newcommand{\tbis}{s}
\newcommand{\tter}{t}

\newcommand{\interval}[2]{\np{{#1}\!:\!{#2}}}
\newcommand{\ic}[1]{\llbracket #1 \rrbracket}
%\newcommand{\inic}[1]{\in \llbracket #1 \rrbracket}
\newcommand{\inic}[2]{=#1,\ldots,#2}

%% Strategies 

\newcommand{\policy}{\lambda}
\newcommand{\Policy}{\Lambda}
\newcommand{\POLICY}{\Lambda}
\newcommand{\strategy}{\policy}
\newcommand{\STRATEGY}{\POLICY}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% VIABILITE
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dec}{\BB} % contraintes_decision
\newcommand{\decset}[1]{\dec\big(#1,x(#1)\big)}
\newcommand{\obj}{\mathbb{D}}
\newcommand{\Uad}{{\cal U}^{\rm ad}} 
\newcommand{\XUad}{{\cal T}^{\rm ad}}
\newcommand{\sdo}{{\mathbb A}} % state domain
\newcommand{\target}{\sdo(\horizon)}

\newcommand{\Ut}{\dec\big(t,\state(t)\big)}
\newcommand{\Us}{\dec(s,\state(s))}
\newcommand{\Utx}{\dec(t,x)}
\newcommand{\Usx}{\dec(s,x)}
\newcommand{\Ux}[1]{\dec^{#1}(\state)}
\newcommand{\UT}[1]{\dec(t,#1)}

\newcommand{\viab}{\mathbb{V}{\rm iab}}
\newcommand{\inv}{{\rm Inv}}
\newcommand{\vviab}{\mbox{\tiny viab}}
\newcommand{\decviab}{\dec^{\vviab}} 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% OPTIMISATION
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\argmin}{\mathop{\arg\min}} 
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
%\renewcommand{\sup}{\max}
%\renewcommand{\inf}{\min}
\newcommand{\Min}{\min}
\newcommand{\Max}{\max}
\newcommand{\MAX}{\max}
\newcommand{\MIN}{\min}

\newcommand{\opt}{^{\star}}             % optimal
\newcommand{\adm}{^{\mbox \rm ad}}      % admissible

\newcommand{\criterion}{j}                                  % Crit\`{e}re
\newcommand{\Criterion}{J}                                  % Crit\`{e}re apres 
\newcommand{\CRITERION}{\tilde{\jmath}} 
   
\newcommand{\coutint}{L}                                    % Co\^{u}t int\'{e}gral
\newcommand{\coutfin}{K}                                    % Co\^{u}t final

\newcommand{\Regret}{r}

\newcommand{\VALUE}{V}
\newcommand{\Value}{V}

\newcommand{\Hamiltonian}{{\cal H}}
\newcommand{\adjoint}{q}

\newcommand{\decrule}{\mathtt{Pol}}
% \usepackage{euscript}
\newcommand{\feedback}[1]{\EuScript{#1}}
\newcommand{\feedbackset}{\EuScript{\Control}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% PROBABILITES
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\prbt}{\mathbb{P}}                              % proba  du triplet
\newcommand{\mathscr}{\EuScript}
\newcommand{\tribu}[1]{\mathscr{#1}}                        % Tribu
\newcommand{\trib}{{\cal F}}
\newcommand{\soustribu}{{\cal G}}
\newcommand{\borel}[1]{\tribu{B}_{#1}^{\mathrm{o}}}

\newcommand{\epro}{(\Omega,\trib,\prbt)}

\newcommand{\va}[1]{\mathbf{#1}}
\newcommand{\RV}{\mathtt{RV}}
\newcommand{\Rv}{\mathtt{Rv}}

\newcommand{\filtration}[1]{\mathbb{#1}}                    % Filtration

%% Probabilit\'{e}

\newcommand{\nprob}[1]{\prbt\normdelim{#1}}                 % Probabilit\'{e} normal
\newcommand{\bprob}[1]{\prbt\bigdelim{#1}}                  % Probabilit\'{e} big
\newcommand{\Bprob}[1]{\prbt\Bigdelim{#1}}                  % Probabilit\'{e} Big
\newcommand{\bgprob}[1]{\prbt\biggdelim{#1}}                % Probabilit\'{e} bigg
\newcommand{\Bgprob}[1]{\prbt\Biggdelim{#1}}                % Probabilit\'{e} Bigg

%% Esp\'{e}rance

\newcommand{\espe}{\mathbb{E}}                              % Symbole
\newcommand{\esper}[1]{\espe\normdelim{#1}}
\newcommand{\expect}[1]{\espe_{#1}}

\newcommand{\nesp}[2][]{\espe_{#1}\nc{#2}}           % Esp\'{e}rance normal
\newcommand{\besp}[2][]{\espe_{#1}\bc{#2}}            % Esp\'{e}rance big
\newcommand{\Besp}[2][]{\espe_{#1}\Bc{#2}}            % Esp\'{e}rance Big
\newcommand{\bgesp}[2][]{\espe_{#1}\bgc{#2}}          % Esp\'{e}rance bigg
\newcommand{\Bgesp}[2][]{\espe_{#1}\Bgc{#2}}          % Esp\'{e}rance Bigg
%
% \newcommand{\nesp}[2][]{\espe_{#1}\normdelim{#2}}           % Esp\'{e}rance normal
% \newcommand{\besp}[2][]{\espe_{#1}\bigdelim{#2}}            % Esp\'{e}rance big
% \newcommand{\Besp}[2][]{\espe_{#1}\Bigdelim{#2}}            % Esp\'{e}rance Big
% \newcommand{\bgesp}[2][]{\espe_{#1}\biggdelim{#2}}          % Esp\'{e}rance bigg
% \newcommand{\Bgesp}[2][]{\espe_{#1}\Biggdelim{#2}}          % Esp\'{e}rance Bigg

%% Esp\'{e}rance conditionnelle

\newcommand{\nespc}[3][]{\espe_{#1}\normdelims{#2}{#3}}     % Esp\'{e}rance cond. normal
\newcommand{\bespc}[3][]{\espe_{#1}\bigdelims{#2}{#3}}      % Esp\'{e}rance cond. big
\newcommand{\Bespc}[3][]{\espe_{#1}\Bigdelims{#2}{#3}}      % Esp\'{e}rance cond. Big
\newcommand{\bgespc}[3][]{\espe_{#1}\biggdelims{#2}{#3}}    % Esp\'{e}rance cond. bigg
\newcommand{\Bgespc}[3][]{\espe_{#1}\Biggdelims{#2}{#3}}    % Esp\'{e}rance cond. Bigg

%% Variance

\newcommand{\vari}{\mathop{\mathsf{var}}}
\newcommand{\cov}{\mathop{\mathsf{cov}}}
\newcommand{\dispersion}{\mathop{\mathsf{D}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% UNCERTITUDES
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\uncertainty}{\omega}
\newcommand{\Uncertainty}{\Omega}
\newcommand{\Om}{\Omega}
\newcommand{\om}{\omega}

\newcommand{\scenario}{s}
\newcommand{\Scenario}{S}
\newcommand{\SCENARIO}{\mathbb{S}}
\newcommand{\Scenarios}{\mathbb{S}}

% \newcommand{\unc{\overline{\UNCERTAIN}}
% \newcommand{\unc{\mathbb S} % constraints domain
% \newcommand{\Unc{\Omega} % contraintes incertitude

\def\scheme{%
\pstree[treemode=R,levelsep=3cm,radius=2pt]{\Tc{2pt}}{%
\pstree{\TC*}{%
\pstree{\TC*}{\Tr{HHH} \Tr{HHC}}
\pstree{\TC*}{\Tr{HCH} \Tr{HCC}}}
\pstree{\TC*}{%
\pstree{\TC*}{\Tr{CHH} \Tr{CHC}}
\pstree{\TC*}{\Tr{CCH} \Tr{CCC}}}}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% MULTI-AGENT
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%PC%%\newcommand{\CRITERION{\tilde{\jmath}}
%%PC%%\newcommand{\Criterion{\overline{\jmath}}
%%PC%%\newcommand{\Qps{\text{${\mathbb Q}$-}\as}

%% Agents 

\newcommand{\agent}{a}
\newcommand{\agentbis}{b}
\newcommand{\agentter}{c}
\newcommand{\agentcuarto}{d}
\newcommand{\AGENT}{A} 

\newcommand{\SubAgents}{B}
\newcommand{\SubAgentsTwo}{C}
\newcommand{\SubAgentsThree}{C'}

\newcommand{\NP}{N}
\newcommand{\player}{p}
\newcommand{\playerbis}{q}
\newcommand{\playerter}{r}
\newcommand{\PLAYER}{P}

\newcommand{\Principal}{\mathtt{Pr}}
\newcommand{\Agent}{\mathtt{Ag}}

%% Sets and fields 

\newcommand{\history}{h}
\newcommand{\History}{H}
\newcommand{\HISTORY}{\mathbb{H}}

\newcommand{\Nature}{N}
\newcommand{\NatureField}{F}

\newcommand{\Decision}{D}
\newcommand{\Information}{I}

%% Relations 

\newcommand{\subsys}{\mathfrak{S}}
\newcommand{\preced}{\mathfrak{P}}
\newcommand{\memory}{\mathfrak{M}}
\newcommand{\decisionmemory}{{\mathfrak{D}}}
\newcommand{\order}{\mathfrak{O}}
\newcommand{\relation}{\mathfrak{R}}
%\newcommand{\partitionfield}{\soustribu}

%% Operations on relations 

\newcommand{\complementary}[1]{{#1}\compl}

\newcommand{\pullback}[1]{\left(#1\right)_{\star}}
\newcommand{\pushback}[1]{\left(#1\right)^{\star}}

\newcommand{\crochet}[1]{\left< #1 \right>_{\preced}}
\newcommand{\bracket}[1]{\left< #1 \right>_{\memory}} 
%\newcommand{\doublecrochet}[1]{\left< #1 \right>_{\decisionmemory}} 

\newcommand{\plusfine}{\succeq}
\newcommand{\moinsfine}{\preceq}

%% Products of sets and fields 

\newcommand{\oproduit}[2]{#2 \otimes #1}
\newcommand{\produit}[2]{#2 \times #1}
\newcommand{\oproduct}[2]{#2 \otimes #1}
\newcommand{\product}[2]{#2 \times #1}
\newcommand{\othreeproduct}[3]{#3 \otimes #2 \otimes #1}
\newcommand{\threeproduct}[3]{#3 \times #2 \times #1}
%
\newcommand{\couple}[2]{\np{#2,#1}}
\newcommand{\bigcouple}[2]{\big(#2,#1\big)}
\newcommand{\Bigcouple}[2]{\Big(#2,#1\Big)}
\newcommand{\bcouple}[2]{\Bp{#2,#1}}
\newcommand{\Bcouple}[2]{\Bp{#2,#1}}
\newcommand{\triplet}[3]{\np{#3,#2,#1}}
\newcommand{\btriplet}[3]{\bp{#3,#2,#1}}
\newcommand{\Btriplet}[3]{\Bp{#3,#2,#1}}

%% 

\newcommand{\hatcontrol}{M} 
\newcommand{\solutionmap}{S} 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                          %%%%%
%%%%% BIOECONOMIE 
%%%%%                                                          %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Biological models 

\newcommand{\mortal}{\mu}
\newcommand{\fertility}{\gamma}
\newcommand{\biomass}{B}
\newcommand{\biology}{\mathtt{Biol}}

%% Economic models 

\newcommand{\interest}{r_{e}} % taux d'intérêt
\newcommand{\discount}{(\frac{1}{1+\interest})}
\newcommand{\Discount}{\frac{1}{1+\interest}}
\newcommand{\DISCOUNT}{\delta}

%\newcommand{\certainty_equiv}{\widehat}

\newcommand{\price}{p}
\newcommand{\effort}{E}
\newcommand{\Effort}{E}
\newcommand{\Catch}{\mathtt{Catch}}
\newcommand{\catch}{h}
\newcommand{\rent}{\mathtt{Rent}}
\newcommand{\profit}{P}
\newcommand{\Production}{\mathtt{Yield}}
\newcommand{\production}{Y}

%% CO2

%\newcommand{\co2}{\textsc{co}$_2$}
%\newcommand{\CO2}{\textsc{co}$_2$}
\newcommand{\ghg}{\textsc{ghg}}
\newcommand{\BAU}{{\rm bau}}
\newcommand{\GWP}{\textsc{gwp}}
\newcommand{\growth}{g}
\newcommand{\Emissions}{\mathtt{Emiss}}
\newcommand{\Damage}{\mathtt{Damage}}

%% Bioeconomic models

\newcommand{\SY}{\mathop{\mathtt{Sust}}}
\newcommand{\MSY}{\textsc{msy}}
\newcommand{\MSE}{\textsc{mse}}
\newcommand{\PPE}{\textsc{ppe}}
\newcommand{\CPE}{\textsc{cpe}}

\newcommand{\Consumption}{\mathtt{Consum}}
\newcommand{\consumption}{C}
\newcommand{\Environment}{\mathtt{Envir}}
\newcommand{\environment}{E}

%% Stock models

\newcommand{\stock}{S}
\newcommand{\volume}{\stock}
\newcommand{\turbined}{q}
\newcommand{\spilled}{r}
\newcommand{\inflow}{a}

\newcommand{\purchasing}{c}
\newcommand{\shortage}{b}
\newcommand{\holding}{h}

%% Fisheries models

\newcommand{\mature}{\gamma}
\newcommand{\weight}{\mu}
\newcommand{\abundance}{N}
\newcommand{\multiplier}{\lambda}
\newcommand{\exploitation}{F}
\newcommand{\mortality}{M}
\newcommand{\SSB}{\mathtt{SSB}}
\newcommand{\spr}{\mathtt{spr}}
%\newcommand{\benefit}{B}

% \newcommand{\spawning_stock_biomass}{{\sf SSB}} 
% \newcommand{\fishing_mortality}{{\sf F}} 
\newcommand{\stockrecruitment}{stock-recruitment} %{{\sf S-R}}
%\renewcommand{\varphi}{\mathtt{S/R}}
\newcommand{\SR}{\mathtt{S/R}}
%\renewcommand{\SR}{\mathop{\mathsf{S/R}}}

\newcommand{\ICES}{\textsc{ices}}
\newcommand{\ices}{{\sf ices}}

\newcommand{\rref}{\llim} %{{\sf ref}}
\newcommand{\Bref}{\Blim} %{B_{{\sf ref}}}
\newcommand{\Fref}{\Flim} %{F_{{\sf ref}}}
\newcommand{\pa}{{\sf pa}}
\newcommand{\Bpa}{B_{\pa}}
\newcommand{\Fpa}{F_{\pa}}
\newcommand{\llim}{{\sf lim}}
\newcommand{\Blim}{B_{\llim}}
\newcommand{\Flim}{F_{\llim}}
\newcommand{\PA}{{\sf PA}}
\newcommand{\LLIM}{\textsc{lim}}
\newcommand{\LPA}{\textsc{pa}}

\newcommand{\ypr}{{\sf ypr}}
\newcommand{\mmin}{{\sf min}}
\newcommand{\mmax}{{\sf max}}
\newcommand{\gm}{{\sf gm}}
\newcommand{\mean}{{\sf mean}}
\newcommand{\msy}{{\sf msy}}

\newcommand{\PVA}{\textsc{pva}}
\newcommand{\CVA}{\textsc{cva}}

\newcommand{\threshold}[1]{{\Violet #1}} 
\newcommand{\equil}{_{\textsc{e}}}

\newcommand{\utility}{\mathtt{L}}
\newcommand{\util}{\mathtt{L}}
\newcommand{\utilfin}{\mathtt{K}}

\newcommand{\cost}{c}
\newcommand{\Cost}{\mathtt{Cost}}
\newcommand{\Costfin}{\mathtt{CostFin}}

\newcommand{\Payoff}{\mathtt{Payoff}}
\newcommand{\payoff}{\mathtt{Payoff}}
\newcommand{\reward}{\mathtt{Reward}}



